Concurrent Reference Counting and Resource Management in Wait-free Constant Time

A common problem when implementing concurrent programs is efficiently protecting against unsafe races between processes reading and then using a resource (e.g., memory blocks, file descriptors, or network connections) and other processes that are concurrently overwriting and then destructing the same resource. Such read-destruct races can be protected with locks, or with lock-free solutions such as hazard-pointers or read-copy-update (RCU). In this paper we describe a method for protecting read-destruct races with expected constant time overhead, $O(P^2)$ space and $O(P^2)$ delayed destructs, and with just single word atomic memory operations (reads, writes, and CAS). It is based on an interface with four primitives, an acquire-release pair to protect accesses, and a retire-eject pair to delay the destruct until it is safe. We refer to this as the acquire-retire interface. Using the acquire-retire interface, we develop simple implementations for three common use cases: (1) memory reclamation with applications to stacks and queues, (2) reference counted objects, and (3) objects manage by ownership with moves, copies, and destructs. The first two results significantly improve on previous results, and the third application is original. Importantly, all operations have expected constant time overhead.

==> alloc.tex <==
Shared Memory Pool supporting allocate and free on memory blocks
of size k in constant time and k(n + O(p^2)) memory, where n is the
maximum number of blocks ever allocated.

Based on chunks each containing p blocks.   A chunk can be kept as a
linked list of blocks using the block memory.
Each processor contains 0 or 1 full chunks, and one partially full chunk
A global stack maintains a stack of full chunks.

****************

Global Stack (basically using a universal construction with multiword ll/sc)
Surely already exists.
 
Push and Pop take O(p) time
I think it takes p^2 space since the ll/sc on objects of size p can take p time

\Hao{For multi-word LL/SC we can use \cite{jayanti2005efficient}. <- Actually 
I don't think this works anymore because they implement $P$ multi-word LL/SC using
$P$ small LL/SC and we would need to use our algorithm to implement $P$ small
LL/SC in the bounds that we want ($P^2$ space, no unbounded seq num, and 
$2\log P$ word size). The easiest thing would probably be to directly use
our own multi-word LL/SC from CAS.}

Data structure

Announce[P] of {None, Push(element), Pop}

struct state { stack s; Response[P] of {None, Pop(element), Push}}

The stack is just a linked list of chunks.  Can use some memory from
the first block in each chunk, but this requires two pointers per
block---one for next in stack, and one for next in chunk.

TryTransition:
LL the state (creates copy and can take p time)
For each i in p
   if announced and not responded, then do operation and insert response
   if responded and not announced, clear response
(All done on local copy of the state and not visible)   
SC the state (can take p time)

Push : announce push in Announce[i], TryTransition twice, clear
          announce, TryTransition twice
	  
Pop : announce pop in Announce[i], TryTransition twice, pull out
          answer, clear announce, TryTransition twice

Deamortize to finishes in p sub-steps each of constant time

****************

Local chunks

Chunks are of size p
The number of full chunks NumChunks is always 1 or 2
Start with 2 full chunks and empty current chunk
NumChunks = 2

Allocate and free from current chunk.
Run deamortized step on each operation.

If allocate empties current chunk then
   current chunk = a local full chunk
   If NumChunks == 1 then
      Delayed Pop to get new full chunk (takes effect within p operations)
   Else 
      NumChunks--

If free fills current chunk then
  if NumChunks == 2 then
    Delayed push of current chunk (takes effect within p operations)
  Else
    move current to full chunk
    NumChunks++
  current chunk = empty

Claim:
Each processor will hold at most 4p elements.  2p in the full chunks,
p in the current chunk, and p delayed on a push.
Will always contain at least one element since takes p steps
operations from taking last chunk, during which time there is a pending pop

*************


==> allocatefree.tex <==
\subsection{Allocate and Free in constant time}

Our goal is to allocate \cfont{allocate} and \cfont{free} for fixed sized objects across a set of $p$ processes.  An \cfont{allocate()} returns a pointer to a block, and a \cfont{free(p)} takes a pointer $p$ to an block.  We say a block is live at some point in time if the last response from an allocation returning the block comes after the last invocation of a free on the block.  As would be expected with allocation, an allocate cannot return a pointer to a live block, and the user can only invoke a free on a live block.  If there are never more than $n$ live blocks our implementation requires $n + O(p^2)$ total blocks.

For a constant $l \in O(p)$ our data structure consists of local private pools that each hold $O(l)$ blocks and a shared pool that maintains a collection of at most $n/l + O(1)$ \emph{batches}, each containing $l$ blocks.  The shared pool is maintained using a shared stack.  Pushes and pops by any process from the shared stack take $O(p)$ time.  However, to deamortize their cost they can be broken into $p$ steps of $O(1)$ time each.  We use a universal construction for the shared stack using standard techniques~\cite{x}.

We manage the private pools as follows.  Each pool has between zero and two full batches with $p$ blocks each.  It also has a current working batch that is partially filled and contain between $1$ and $p-1$ elements, and possibly one of either a poped batch or a pushed batch from the shared pool that are currently being processed.  Due to the deamortization, the batches from the shared pool will complete $p$ operations after they start.  We maintain a NumBatches variable that presents the number of full batches plus one if there is a pop currently being processed (started but not completed).  This variable always has a value of 1 or 2.  The pseudocode for allocate and free is given in Figure~\ref{fig:allocfree}.

\begin{figure}
\small
\begin{verbatim}
using batch = stack<block>;
shared_stack<batch> shared_pool;
thread_local stack<batch> local_batches; 
thread_local stack<block> current_batch;
int num_batches = 2;

block* allocate() {
  if (current_batch.empty()) {
    current_batch = local_batches.pop();
    if (num_batches == 1) 
      delayed local_batches.push(shared_pool.pop());
    else num_batches--;
  }
  run_delayed_step();
  return current_batch.pop();
}

void free(block* b) {
  if (current_batch.full()) {
    if (num_batches == 2) 
      delayed shared_pool.push(current_batch);
    else {
      num_batches++;
      local_batches.push(current_batch);
    }
    current_batch = empty;
  }
  run_delayed_step();
  current_batch.push(b);
}
\end{verbatim}
\caption{Allocation anf Free}
\label{fig:allocfree}
\end{figure}

Claim:
Each processor will hold at most 4p elements.  2p in the full chunks,
p in the current chunk, and p delayed on a push.
Will always contain at least one element since takes p steps
operations from taking last chunk, during which time there is a pending pop


==> atomic_copy.tex <==
\section{Atomic Copy}

\Hao{copy can also apply an arbitrary function.}

  \renewcommand{\figurename}{Algorithm}
  \begin{figure}[!t!h]
  \caption{Atomic copy (single-writer)}
  \begin{lstlisting}[linewidth=\columnwidth]

struct data_t {
  union val_or_ptr_t {
    value_t val;
    value_t* ptr;
  }
  state_t state; // either copying or done
}

struct copyable_t {
  data_t data; // LL/SC object
  value_t old;
}

// dest is single writer
void copy(value_t *src, copyable_t *dest) {
  dest->old = dest->data.val;
  dest->data = <src, copying>;
  value_t val = *src;
  CAS(&(dest->data), <src, copying>, 
                     <val, done>);
}

value_t read(copyable_t *x) {
  optional<data_t> c = LL_weak(&(x->data));
  if(c == empty) {
    c = LL_weak(&(x->data));
    if(c == empty) return x->old;
  }
  // c is guaranteed to be not empty
  if(c.state == copying)
  {
    value_t val = *(c.ptr);
    if(SC(&(x->data), <val, done>))
      return val;
    else
      return x->old;
  }
  else return c.val;
}

value_t write(copyable_t *x, value_t new_val) {
  dest->data.val = new_val;
}
  \end{lstlisting}
  \label{alg:rwcas}
  \end{figure}
  \renewcommand{\figurename}{Figure}

